Causal Strategic Learning with Competitive Selection

We study the problem of agent selection in causal strategic learning under multiple decision makers and address two key challenges that come with it. Firstly, while much of prior work focuses on studying a fixed pool of agents that remains static regardless of their evaluations, we consider the impact of selection procedure by which agents are not only evaluated, but also selected. When each decision maker unilaterally selects agents by maximising their own utility, we show that the optimal selection rule is a trade-off between selecting the best agents and providing incentives to maximise the agents' improvement. Furthermore, this optimal selection rule relies on incorrect predictions of agents' outcomes. Hence, we study the conditions under which a decision maker's optimal selection rule will not lead to deterioration of agents' outcome nor cause unjust reduction in agents' selection chance. To that end, we provide an analytical form of the optimal selection rule and a mechanism to retrieve the causal parameters from observational data, under certain assumptions on agents' behaviour. Secondly, when there are multiple decision makers, the interference between selection rules introduces another source of biases in estimating the underlying causal parameters. To address this problem, we provide a cooperative protocol which all decision makers must collectively adopt to recover the true causal parameters. Lastly, we complement our theoretical results with simulation studies. Our results highlight not only the importance of causal modeling as a strategy to mitigate the effect of gaming, as suggested by previous work, but also the need of a benevolent regulator to enable it.

==> sections/00_storyline.tex <==

%\section*{Storyline}
%\begin{enumerate}
%    \item \textbf{Overarching message.} 
%    We show that in the setting where decision makers selfishly select agents, their optimal decision rules are a trade off between selecting the best agents and incentivising everyone, thus it might harm the society if the majority of the population is discouraged from improving. Therefore, we provide some conditions a social planner could impose to mitigate the harm on the society.
%    \item Starting from a single decision maker~(DM) that is a utility maximiser, we show that the optimal solution $\thetaao = A + \mathcal{E}\mathcal{E}^\top\thetastar$ can be interpreted as DM having the freedom to design selection rule that either prefers selecting student with better baseline or putting more effort in incentivizing the others. {\color{red}If we assume the latter is more costly than the former, it is fair to say that DM has the incentive to select smarter students, instead of incentivizing the population.} The optimal solution however can be estimated without the need for causal estimation. \Krik{Let's make it a little bit more dramatic. What would the society looks like if the decision maker adopts an optimal solution $\thetaao$ that is different from the true causal parameter $\thetastar$?} \Kiet{Done, below.}
%    If the decision maker adopts an optimal solution $\thetaao$ that does not align with $\mathcal{E}\mathcal{E}^\top\thetastar$, this leads to deterioration in agents' potential outcomes. In reality, this can be thought of as the best agents have little incentive to improve further if they know that they are likely to be selected (i.e., negative cPI) and/or mediocre agents have little incentive to improve if they know they have little chance to be selected (e.g., negative mPI).
%    \item Now come in from the angle of a regulator whose goal is to ensure positive improvement of agents' outcomes. As such, this regulator will impose an alignment rule where "the resulting vector $\{A+\mathcal{E}\mathcal{E}^\top\bm{\theta}^*\}$ has to point in the same direction as $\mathcal{E}\mathcal{E}^\top\bm{\theta}^*$", to achieve this, we need to estimate $\mathcal{E}\mathcal{E}^\top\bm{\theta}^*$. The regulator proposes an algorithm for this single decision maker to recover the true causal parameters $\thetastar$ under selection bias, by releasing scaled duplicates of decision parameters. The decision maker can then compute $\mathcal{E}\mathcal{E}^\top\thetastar$ and subsequently design a selection rule such that $A$ satisfies the alignment rule. 
%    \Krik{And make it clear what the new contributions are (e.g., we elucidate what the regulator should do).} \Kiet{Done, above.}
    
%    (In appendix: Our estimation procedure can also be trivially adjusted to \textit{directly} estimate $\mathcal{E}\mathcal{E}^\top\bm{\theta}^*$, but we do not want that because having access to $\bm{\theta}^*$ is useful for investigating other decision making objectives as well, such as robustness \cite{shavit2020causal} and fairness \cite{harris2022strategic}.)

%    Moreover, the admission chance of agent might be unjustly decreased if a decision maker selfishly employs his/her optimal decision parameters $\thetaao$ instead of the true causal parameters $\thetastar$. We propose some conditions a regulator can impose to safeguard this admission chance from decreasing when the decision maker uses $\thetaao$ instead of $\thetastar$. \footnote{This result does not assume any specific selection rule besides the fact that it must be monotonic to the prediction.}
    
%    \item We now extend to a more \textit{realistic} scenario where there are multiple decision makers selecting from the same pool of agents, thus requiring additional assumptions and conditions to arrive at the same solutions in the single-DM setting. We introduce an assumption to obtain the dominant strategy $\bm{\theta}_i^\text{AO}$ for an arbitrary decision-maker $i$. We mention that this optimal decision rule is also a trade-off between selecting the best and incentivising everyone. \Krik{This part appears disconnected from the previous two parts.} \Kiet{Done, editted.}
%    \item If the regulator wants to safeguard the social welfare again, which requires the alignment rule, then a faithful estimation of $\bm{\theta}_j^*$ (or $\mathcal{E}\mathcal{E}^\top\bm{\theta}_j^*$) for every DM $j$ where $j=1,\ldots,n$ is needed. The regulator, in addition, proposes a collaborative protocol where all DMs must release scaled duplicates synchronously in order to obtain better causal estimation.
%    \Krik{Now, it becomes unclear how the strategic behaviours of the agents come into the picture.}
%    \Kiet{The strategic behaviour of agents gives rise to the improvement part, $\bm{\theta}^\top\mathcal{E}\mathcal{E}^\top\thetastar$. When there is no strategic behaviour, there is no improvement, optimal selection rule amounts to just selecting the best.}
%    Similarly, we provide additional conditions for the regulator to safeguard the admission chance of an agent, with respect to all decision makers.
%\end{enumerate}

